When Youth Enter the Algorithmic Wild: Discovering and Understanding Potentially Harmful Teen Videos on Douyin and Kwai

Short-video platforms like Douyin and Kwai have become central to adolescent digital life, but they also risk exposing teens to algorithmically amplified harmful content. Despite its societal importance, the scale, mechanisms, and real-world impact of this exposure remain poorly understood. Measuring it is challenging: recommendation feeds are personalized black boxes, harmful content employs sophisticated evasion tactics, and naive crawlers fail to replicate authentic teen behavior. To bridge this gap, we propose PHTV-Scout, the first large-scale, behaviorally grounded measurement framework for Potentially Harmful Teen Videos (PHTVs). We integrate an offline survey of 683 adolescents with a tri-module online pipeline: (1) PHTV Hunter simulates teen accounts to collect recommendation feeds; (2) PHTV Arbiter, a LoRA-finetuned multimodal classifier, detects PHTVs with 94.29% accuracy and 96.41% precision; and (3) PHTV Analyzer performs fine-grained categorization and impact assessment. Over six months, we analyzed 186,727 videos and 51,287 comments, uncovering a troubling 6.11% PHTV prevalence--dominated by Child Sexual Exploitation Imagery (53.2%)--and revealing that harmful content thrives through covert interactions (e.g., grooming comments, self-disclosure) and active evasion (semantic camouflage, noise injection). Crucially, while Youth Mode blocks 100% of PHTVs, its low adoption (30-41%) leaves most teens unprotected. We further show that exposure is driven not by user identity but by regulation, platform algorithms, and even passive browsing, exposing the fragility of adolescent information environments. Our findings call for a paradigm shift from reactive takedowns to proactive, human-centered safeguards.

==> 0_title.tex <==
\title{Harmful Teen Videos on Douyin and Kwai: Landscape, Evolution, and Negative Impact}
\title{Shadows in the Scroll: Unveiling the Landscape of Potentially Harmful Teen Videos on Douyin and Kwai}
\title{Dark Patterns and Dangerous Feeds:A Large-Scale Agentic Characterization of Teen-At-Risk Content on Douyin and Kwai}
\title{PHTV-Hunter: Agentic Discovery and Characterization of Potentially Harmful Teen Videos on Douyin and Kwai}
\title{The Youth Mode Paradox: Measuring the Gap Between Technical Safeguards and Real-World Exposure to Harmful Content on Short-Video Platforms}
\title{When Safety Isn’t Used: Measuring the Real-World Gap Between Platform Safeguards and Teen Exposure to Harmful Short Videos}
\title{When Youth Enter the Wild of Short Videos: Discovering and Understanding Potentially Harmful Teen Videos on Short-Video Platforms}
\title{Measuring Harm in the Algorithmic Wild: Discovering and Characterizing Potentially Harmful Teen Videos on Douyin and Kwai}
\title{When Youth Enter the Wild of Short Videos: Discovering and Understanding Potentially Harmful Teen Videos on Douyin and Kwai}
\title{When Youth Enter the Algorithmic Wild: Discovering and Understanding Potentially Harmful Teen Videos on Douyin and Kwai}

==> commons/pkgs.tex <==
% \usepackage[utf8]{inputenc}
\usepackage{CJKutf8}
% it, be sure to load this package with the cmex10 option to ensure that
% only type 1 fonts will utilized at all point sizes. Without this option,
% it is possible that some math symbols, particularly those within
% footnotes, will be rendered in bitmap form which will result in a
% document that can not be IEEE Xplore compliant!
\usepackage{amsmath}
\usepackage{graphicx}
% it is a good idea to load it with the tight package option to reduce
% the amount of white space around the subfigures. 
\usepackage[tight,footnotesize]{subfigure}
%\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage{multirow}
\usepackage{fancyvrb}
\usepackage[flushleft, online]{threeparttable}
% Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space,


% \usepackage{cite}
% % \usepackage{url}
%  % \usepackage[hyphens]{url}
%  \usepackage{xurl}
% \usepackage{array}
% \usepackage{algorithmic}
% \usepackage{booktabs}
% \usepackage{xcolor}
% \usepackage{ulem}
% \usepackage{authblk}
% \usepackage[
%     colorlinks,
%     linkcolor=blue,
%     anchorcolor=blue,
%     citecolor=blue,
%     urlcolor=blue
% ]{hyperref}

\ifdefined\ccs
\else
    \usepackage{cite}
\fi
\usepackage{xurl}
\usepackage{array}
\usepackage{algorithmic}
\usepackage{booktabs}
\usepackage{xcolor}
\usepackage{CJKutf8}
% \usepackage{authblk}

% \usepackage{emoji}
% \usepackage{twemoji}
% \usepackage{fontspec}
\usepackage[normalem]{ulem}

==> sections/10_ethical.tex <==
\section*{Ethical Considerations}
\label{appendix:ethical_considerations}

\subject{Stakeholders.}
Our research involves multiple stakeholders, including (1) adolescent participants in our offline survey, (2) their legal guardians, (3) the two participating schools (a middle school and a high school), (4) platform users on Kwai and Douyin (including content creators and viewers), (5) the platforms themselves (Kuaishou and Douyin), (6) policymakers, (7) educators, and (8) the broader public concerned with youth digital safety. (9) The research team is also a stakeholder, responsible for ethical data handling and scientific integrity.

\subject{Impacts.}
We considered the following ethical principles from \textit{The Menlo Report}: \textbf{Beneficence}, \textbf{Respect for Persons}, \textbf{Justice}, and \textbf{Respect for Law and Public Interest}.

\noindent\textbf{Harms} include:  
(1) Questions in user studies may make participating teenagers uncomfortable;
(2) potential re-identification or psychological distress if raw video/comment data were leaked;  
(3) unintended amplification of harmful content during account mimicking (e.g., through likes or shares);  
(4) misinterpretation of benign content as harmful due to classification errors;
(5) although our synthetic accounts mimic real teens, they do not represent actual users, raising concerns about representativeness if findings are overgeneralized; and
(6) psychological risks to research team members and annotators who review harmful content during the labeling process.

\subject{Mitigations.}
To address these risks, we implemented multiple safeguards:
\begin{itemize}
    \item \textbf{Questionnaire Design:} The questionnaires used for user surveys were carefully designed to minimize any potential discomfort (see Appendix~\ref{app:questionnaire_full}). The questionnaire clearly stated that participation in this study was entirely voluntary, anonymous, and carried an extremely low risk. No personally identifiable information (such as name, student ID, or phone number) was collected. All data is stored on an encrypted local server, accessible only to research team members, and will be securely deleted after two years.
    
    \item \textbf{Institutional Oversight:} The offline user study received approval from both participating schools, and all participants (and their legal guardians) signed dual-party informed consent forms (see Appendix~\ref{app:consent_form}). The form explicitly stated the low-risk nature of participation and guaranteed anonymity. Our institution does not currently maintain a dedicated IRB-style process for this category of internet measurement and school-based survey work. In the absence of such a mechanism, we followed a documented ethics process grounded in AoIR guidance, school approval, national minor-protection requirements, and ongoing internal risk review.
    
    \item \textbf{Data Minimization \& Anonymization:} We collect only publicly available content from recommendation feeds. All video and comment data are stripped of metadata that could link to specific users and stored on an encrypted, access-controlled server. Raw videos are retained only for validation and will be permanently deleted after publication. We will not release raw video or audio files; any released artifact will be restricted to de-identified, non-invertible, research-oriented representations and documentation, accompanied by content warnings and use restrictions.
    
    \item \textbf{Passive Crawling Protocol:} Our accounts, once set up, perform strictly passive consumption---no likes, comments, shares, or searches are executed---eliminating any risk of algorithmic amplification or engagement with harmful content. This design choice accepts some loss of ecological realism in order to avoid engagement actions that could amplify harmful content.
    
    \item \textbf{Careful Data Collection:} Our data collection on Kwai and Douyin is designed to comply with platform policies and our measurement methodology follows best ethic practices with risks minimized. Particularly, data collection simulated legitimate user behavior using official APIs and rate-limiting delays were enforced to avoid server overload. Besides, content analysis was strictly limited to aggregating statistics and locating predictive insights. All data handling, including the storage of videos and comments, follows protocols for secure and confidential research data management.
    
    \item \textbf{Human-in-the-Loop Validation:} All model-based classifications (binary and multi-class) undergo manual spot-checking by trained annotators. Harmful content examples presented in the paper are fully anonymized (e.g., blurred faces, redacted text). We agree that even blurred screenshots may create reverse-image-search or re-identification risk; therefore, we have removed such images from this version and replaced them with anonymized textual descriptions.
    
    \item \textbf{Responsible Disclosure:} Findings related to platform-specific vulnerabilities (e.g., evasion tactics, timing strategies) are reported at an aggregate level without exposing individual creators or enabling the replication of harmful content. We focused on aggregate disclosure and platform reporting pathways rather than exposing individual creators in the paper. This choice was intended to reduce the risk of harassment, misidentification, and unnecessary secondary harm while still surfacing systemic safety problems.
    
    \item \textbf{Researcher Wellbeing:} Reviewing harmful content poses psychological risks to annotators and researchers. Annotators were informed in advance about the nature of the material, could stop at any time without penalty, worked under capped session lengths (maximum two hours) with mandatory breaks, held debriefs for difficult cases, and had access to institutional counseling support. We established a referral path to university counseling resources for any team member experiencing distress.
    
    \item \textbf{Handling Potentially Illegal Content:} Our taxonomy is intended to study potentially harmful content, not to collect or retain material that is illegal under applicable law. If annotators encountered content suspected of crossing that boundary, they stopped labeling immediately, isolated the case under restricted access, and used the platform's official reporting channel. Such content was not retained as part of the sharable research dataset.
\end{itemize}

\subject{Key Ethical Trade-offs.}
Our study involved several ethical trade-offs that we explicitly acknowledge:

\noindent\textbf{Passive measurement vs. realism.} We accepted some loss of ecological realism in order to avoid engagement actions that could amplify harmful content.

\noindent\textbf{Reproducibility vs. data minimization.} We retained only what was necessary for validation and reproducibility, under encrypted and access-controlled storage, while limiting future sharing to de-identified artifacts.

\noindent\textbf{Systemic reporting vs. individual reporting.} We focused on aggregate disclosure and platform reporting pathways rather than exposing individual creators in the paper. This choice was intended to reduce the risk of harassment, misidentification, and unnecessary secondary harm while still surfacing systemic safety problems.

\subject{Dataset Size and Composition.}
Two datasets served different purposes in our study. The annotated ground-truth set was expanded until the annotation process stopped yielding meaningfully new harmful subtypes. The larger passive measurement corpus was needed to estimate exposure rates and observe lower-frequency patterns such as evasion behaviors. We applied data minimization principles throughout, retaining only content necessary for validation and aggregate analysis.


==> sections/pic.tex <==
\todoVone{Add sections to the \texttt{sections} dir}
\todoVone{Add sections to the \texttt{sections} dir}
\todoVone{Add bibtex entries into the \texttt{ref.bib} file}
\todoVone{Place figures into the \texttt{figures} dir}
\todoVtwo{Further improve this template with more custom features and commands}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{Subfigure 1}
        \label{fig:subfig1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{Subfigure 2}
        \label{fig:subfig2}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{Subfigure 3}
        \label{fig:subfig3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{example-image}
        \caption{Subfigure 4}
        \label{fig:subfig4}
    \end{subfigure}
    \caption{A figure with four subfigures (example images).}
    \label{fig:four-subfigures}
\end{figure}
